RIS-Assisted High Resolution Radar Sensing

This paper analyzes monostatic sensing by a user equipment (UE) for a setting in which the UE is unable to resolve multiple targets due to their interference within a single resolution bin. It is shown how sensing accuracy, in terms of both detection rate and localization accuracy, can be boosted by a reconfigurable intelligent surface (RIS), which can be advantageously used to provide signal diversity and aid in resolving the targets. Specifically, assuming prior information on the presence of a cluster of targets, a RIS beam sweep procedure is used to facilitate the high resolution sensing. We derive the Cram\'er-Rao lower bounds (CRLBs) for channel parameter estimation and sensing and an upper bound on the detection probability. The concept of coherence is defined and analyzed theoretically. Then, we propose an orthogonal matching pursuit (OMP) channel estimation algorithm combined with data association to fuse the information of the non-RIS signal and the RIS signal and perform sensing. Finally, we provide numerical results to verify the potential of RIS for improving sensor resolution, and to demonstrate that the proposed methods can realize this potential for RIS-assisted high resolution sensing.

==> bib/mybib.tex <==
@book{Bourdoux2020,
    author = {Bourdoux, Andre and Barreto, Andre Noll and van Liempd, Barend and de Lima, Carlos and Dardari, Davide and Belot, Didier and Lohan, Elana-Simona and Seco-Granados, Gonzalo and Sarieddeen, Hadi and Wymeersch, Henk and Suutala, Jaakko and Saloranta, Jani and Guillaud, Maxime and Isomursu, Minna and Valkama, Mikko and Aziz, Muhammad Reza Kahar and Berkvens, Rafael and Sanguanpuak, Tachporn and Svensson, Tommy and Miao, Yang},
    title = {{6G} White Paper on Localization and Sensing},
    publisher = {arXiv},
    year = {2020},
}

@article{Liu2022,
    author={Liu, Fan and Cui, Yuanhao and Masouros, Christos and Xu, Jie and Han, Tony Xiao and Eldar, Yonina C. and Buzzi, Stefano},
    journal={IEEE J. Sel. Areas Commun.}, 
    title={Integrated Sensing and Communications: Toward Dual-Functional Wireless Networks for {6G} and Beyond}, 
    year={2022},
    volume={40},
    number={6},
    pages={1728-1767},
    doi={10.1109/JSAC.2022.3156632}
}

@article{Bjornson2022,
    author={Bj\"ornson, Emil and Wymeersch, Henk and Matthiesen, Bho and Popovski, Petar and Sanguinetti, Luca and de Carvalho, Elisabeth},
    journal={IEEE Signal Process. Mag.}, 
    title={Reconfigurable Intelligent Surfaces: A signal processing perspective with wireless applications}, 
    year={2022},
    volume={39},
    number={2},
    pages={135-158},
    doi={10.1109/MSP.2021.3130549}
}

@article{Chen2023:Smart,
    author={Chen, Hui and Kim, Hyowon and Ammous, Mustafa and Seco-Granados, Gonzalo and Alexandropoulos, George C. and Valaee, Shahrokh and Wymeersch, Henk},
    journal={IEEE Commun. Mag.}, 
    title={{RISs} and Sidelink Communications in Smart Cities: The Key to Seamless Localization and Sensing}, 
    year={2023},
    volume={61},
    number={8},
    pages={140-146},
    doi={10.1109/MCOM.001.2200970}
}

@article{Wymeersch2020,
    author={Wymeersch, Henk and He, Jiguang and Denis, Benoit and Clemente, Antonio and Juntti, Markku},
    journal={IEEE Veh. Technol. Mag.}, 
    title={Radio Localization and Mapping With Reconfigurable Intelligent Surfaces: Challenges, Opportunities, and Research Directions}, 
    year={2020},
    volume={15},
    number={4},
    pages={52-61},
    doi={10.1109/MVT.2020.3023682}
}

@article{Aubry2021Surveillance,
    author={Aubry, Augusto and De Maio, Antonio and Rosamilia, Massimo},
    journal={IEEE Trans. Veh. Technol.}, 
    title={Reconfigurable Intelligent Surfaces for {N-LOS} Radar Surveillance}, 
    year={2021},
    volume={70},
    number={10},
    pages={10735-10749},
    doi={10.1109/TVT.2021.3102315}
}

@article{Zhang2022Ubiquitous,
    author={Zhang, Hongliang and Di, Boya and Bian, Kaigui and Han, Zhu and Poor, H. Vincent and Song, Lingyang},
    journal={Proc. IEEE}, 
    title={Toward Ubiquitous Sensing and Localization With Reconfigurable Intelligent Surfaces}, 
    year={2022},
    volume={110},
    number={9},
    pages={1401-1422},
    doi={10.1109/JPROC.2022.3169771}
}

@inproceedings{Keykhosravi2022,
    author={Keykhosravi, Kamran and Seco-Granados, Gonzalo and Alexandropoulos, George C. and Wymeersch, Henk},
    booktitle={2022 IEEE Int. Conf. Commun.}, 
    title={{RIS}-Enabled Self-Localization: Leveraging Controllable Reflections With Zero Access Points}, 
    year={2022},
    volume={},
    number={},
    pages={2852-2857},
    doi={10.1109/ICC45855.2022.9839225}
}

@article{Yang2022MetaSLAM,
    author={Yang, Ziang and Zhang, Haobo and Zhang, Hongliang and Di, Boya and Dong, Miaomiao and Yang, Lu and Song, Lingyang},
    journal={IEEE Trans. Wirel. Commun.}, 
    title={{MetaSLAM}: Wireless Simultaneous Localization and Mapping Using Reconfigurable Intelligent Surfaces}, 
    year={2022},
    volume={},
    number={},
    pages={1-1},
    doi={10.1109/TWC.2022.3213053}
}

@article{Mahler2003Multitarget,
    author={Mahler, R.P.S.},
    journal={IEEE Trans. Aerosp. Electron. Syst.}, 
    title={Multitarget Bayes filtering via first-order multitarget moments}, 
    year={2003},
    volume={39},
    number={4},
    pages={1152-1178},
    doi={10.1109/TAES.2003.1261119}
}

@inproceedings{Clark2006GMPHD,
    author={Clark, Daniel E. and Panta, Kusha and Vo, Ba-ngu},
    booktitle={2006 9th International Conference on Information Fusion}, 
    title={The {GM-PHD} Filter Multiple Target Tracker}, 
    year={2006},
    volume={},
    number={},
    pages={1-8},
    doi={10.1109/ICIF.2006.301809}
}

@article{Hue2002fusion,
    author={Hue, C. and Le Cadre, J.-P. and Perez, P.},
    journal={IEEE Trans. Signal Process.}, 
    title={Sequential Monte Carlo methods for multiple target tracking and data fusion}, 
    year={2002},
    volume={50},
    number={2},
    pages={309-325},
    doi={10.1109/78.978386}
}

@article{Vo2006GMPHD,
    author={Vo, B.-N. and Ma, W.-K.},
    journal={IEEE Trans. Signal Process.}, 
    title={The Gaussian Mixture Probability Hypothesis Density Filter}, 
    year={2006},
    volume={54},
    number={11},
    pages={4091-4104},
    doi={10.1109/TSP.2006.881190}
}

@article{Mahler2007Higher,
    author={Mahler, R.P.S.},
    journal={IEEE Trans. Aerosp. Electron. Syst.}, 
    title={{PHD} filters of higher order in target number}, 
    year={2003},
    volume={43},
    number={4},
    pages={1523 - 1543},
    doi={10.1109/TAES.2007.4441756}
}

@book{Mahler2007Fusion,
    author = {Mahler, Ronald P. S.},
    title = {Statistical Multisource-Multitarget Information Fusion},
    year = {2007},
    isbn = {1596930926},
    publisher = {Artech House, Inc.},
    address = {USA}
}

@article{Fernandez2018PMBM,
    author={Garc\'ia-Fern\'andez, \'Angel F. and Williams, Jason L. and Granstr\"om, Karl and Svensson, Lennart},
    journal={IEEE Trans. Aerosp. Electron. Syst.}, 
    title={Poisson Multi-Bernoulli Mixture Filter: Direct Derivation and Implementation}, 
    year={2018},
    volume={54},
    number={4},
    pages={1883-1901},
    doi={10.1109/TAES.2018.2805153}
}

@inproceedings{Septier2009MCMC,
    author={Septier, François and Pang, Sze Kim and Carmi, Avishy and Godsill, Simon},
    booktitle={2009 3rd IEEE International Workshop on Computational Advances in Multi-Sensor Adaptive Processing (CAMSAP)}, 
    title={On {MCMC}-Based particle methods for Bayesian filtering: Application to multitarget tracking}, 
    year={2009},
    volume={},
    number={},
    pages={360-363},
    doi={10.1109/CAMSAP.2009.5413256}
}

@article{Li2023NHPP,
    author={Li, Qing and Gan, Runze and Liang, Jiaming and Godsill, Simon J.},
    journal={IEEE Trans. Signal Process.}, 
    title={An Adaptive and Scalable Multi-Object Tracker Based on the Non-Homogeneous Poisson Process}, 
    year={2023},
    volume={71},
    number={},
    pages={105-120},
    doi={10.1109/TSP.2023.3240498}
}

@inproceedings{Gan2022Variational,
    author={Gan, Runze and Li, Qing and Godsill, Simon},
    booktitle={2022 25th International Conference on Information Fusion (FUSION)}, 
    title={A Variational Bayes Association-based Multi-object Tracker under the Non-homogeneous Poisson Measurement Process}, 
    year={2022},
    volume={},
    number={},
    pages={1-8},
    doi={10.23919/FUSION49751.2022.9841303}
}

@article{Meyer2021Tracking,
    author={Meyer, Florian and Williams, Jason L.},
    journal={IEEE Trans. Signal Process.}, 
    title={Scalable Detection and Tracking of Geometric Extended Objects}, 
    year={2021},
    volume={69},
    number={},
    pages={6283-6298},
    doi={10.1109/TSP.2021.3121631}
}

@article{Koch2008RandomMatrices,
    author={Koch, Johann Wolfgang},
    journal={IEEE Trans. Aerosp. Electron. Syst.}, 
    title={Bayesian approach to extended object and cluster tracking using random matrices}, 
    year={2008},
    volume={44},
    number={3},
    pages={1042-1059},
    doi={10.1109/TAES.2008.4655362}
}

@inproceedings{Hyowon2023:Bounce,
    author={Kim, Hyowon and Fascista, Alessio and Chen, Hui and Ge, Yu and Alexandropoulos, George C. and Seco-Granados, Gonzalo and Wymeersch, Henk},
    booktitle={2023 IEEE Int. Conf. Commun. Workshops}, 
    title={{RIS}-Aided Monostatic Sensing and Object Detection with Single and Double Bounce Multipath}, 
    year={2023},
    volume={},
    number={},
    pages={1883-1889},
    doi={10.1109/ICCWorkshops57953.2023.10283494}
}

@article{Buzzi2022Radar,
    author={Buzzi, Stefano and Grossi, Emanuele and Lops, Marco and Venturino, Luca},
    journal={IEEE Trans. Signal Process.}, 
    title={Foundations of {MIMO} Radar Detection Aided by Reconfigurable Intelligent Surfaces}, 
    year={2022},
    volume={70},
    number={},
    pages={1749-1763},
    doi={10.1109/TSP.2022.3157975}
}

@article{Keykhosravi2022SISO,
    author={Keykhosravi, Kamran and Keskin, Musa Furkan and Seco-Granados, Gonzalo and Popovski, Petar and Wymeersch, Henk},
    journal={IEEE Journal of Selected Topics in Signal Processing}, 
    title={{RIS}-Enabled {SISO} Localization Under User Mobility and Spatial-Wideband Effects}, 
    year={2022},
    volume={16},
    number={5},
    pages={1125-1140},
    doi={10.1109/JSTSP.2022.3175036}
}

@book{Keykhosravi2021Multi,
    title = {Multi-{RIS} Discrete-Phase Encoding for Interpath-Interference-Free Channel Estimation},
    author = {Keykhosravi, Kamran and Wymeersch, Henk},
    publisher = {arXiv},
    year = {2021},
}

@article{Chen2024:Sidelink,
    author={Chen, Hui and Zheng, Pinjun and Keskin, Musa Furkan and Al-Naffouri, Tareq and Wymeersch, Henk},
    journal={IEEE Trans. Wirel. Commun.}, 
    title={Multi-{RIS}-Enabled {3D} Sidelink Positioning}, 
    year={2024},
    volume={},
    number={},
    pages={1-1},
    doi={10.1109/TWC.2024.3353387}
}

@book{Moeller2003,
    author = {Jesper Moeller and Rasmus Plenge Waagepetersen},
    title = {Statistical Inference and Simulation for Spatial Point Processes },
    year = {2003},
    edition = {1st ed.},
    publisher = {Chapman and Hall/CRC},
    doi = {10.1201/9780203496930}
}

@book{Lieshout2000,
    author = {van Lieshout, M N M},
    title = {Markov Point Processes and Their Applications},
    publisher = {Imperial College Press},
    year = {2000},
    doi = {10.1142/p060}
}

@article{Kopecky2016Bayesian,
    author={Kopeck\'y, Ji\v{r}\'i and Mrkvi\v{c}ka, Tom\'a\v{s}},
    journal={Applications of Mathematics}, 
    title={On the Bayesian estimation for the stationary Neyman-Scott point processes}, 
    year={2016},
    volume={61},
    number={},
    pages={503-514},
    doi={10.1007/s10492-016-0144-8}
}

@article{Tierney1998Metropolis,
     issn = {10505164},
     author = {Luke Tierney},
     journal = {The Annals of Applied Probability},
     number = {1},
     pages = {1--9},
     publisher = {Institute of Mathematical Statistics},
     title = {A Note on Metropolis-Hastings Kernels for General State Spaces},
     volume = {8},
     year = {1998}
}

@article{AbuShaban2018Bounds,
    author={Abu-Shaban, Zohair and Zhou, Xiangyun and Abhayapala, Thushara and Seco-Granados, Gonzalo and Wymeersch, Henk},
    journal={IEEE Trans. Wirel. Commun.}, 
    title={Error Bounds for Uplink and Downlink {3D} Localization in {5G} Millimeter Wave Systems}, 
    year={2018},
    volume={17},
    number={8},
    pages={4939-4954},
    doi={10.1109/TWC.2018.2832134}
}

@article{Shahmansoori2018,
    author={Shahmansoori, Arash and Garcia, Gabriel E. and Destino, Giuseppe and Seco-Granados, Gonzalo and Wymeersch, Henk},
    journal={IEEE Trans. Wirel. Commun.}, 
    title={Position and Orientation Estimation Through Millimeter-Wave {MIMO} in {5G} Systems}, 
    year={2018},
    volume={17},
    number={3},
    pages={1822-1835},
    doi={10.1109/TWC.2017.2785788}
}

@article{Xue2021DBSCAN,
    author={Xue, Xirui and Huang, Shucai and Xie, Jiahao and Ma, Jiashun and Li, Ning},
    journal={IEEE Access}, 
    title={Resolvable Cluster Target Tracking Based on the {DBSCAN} Clustering Algorithm and Labeled {RFS}}, 
    year={2021},
    volume={9},
    number={},
    pages={43364-43377},
    doi={10.1109/ACCESS.2021.3066629}
}

@article{Moeller2005GeneralisedShotNoise,
    ISSN = {00018678},
    author = {Jesper Møller and Giovanni Luca Torrisi},
    journal = {Advances in Applied Probability},
    number = {1},
    pages = {48--74},
    publisher = {Applied Probability Trust},
    title = {Generalised Shot Noise Cox Processes},
    volume = {37},
    year = {2005}
}

@article{He2018Tracking,
    author={He, Shaoming and Shin, Hyo-Sang and Tsourdos, Antonios},
    journal={IEEE Sensors Journal}, 
    title={Multi-Sensor Multi-Target Tracking Using Domain Knowledge and Clustering}, 
    year={2018},
    volume={18},
    number={19},
    pages={8074-8084},
    doi={10.1109/JSEN.2018.2863105}
}

@inproceedings{Li2022Scalable,
    author={Li, Qing and Liang, Jiaming and Godsill, Simon},
    booktitle={ICASSP 2022 - 2022 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, 
    title={Scalable Data Association and Multi-Target Tracking Under a Poisson Mixture Measurement Process}, 
    year={2022},
    volume={},
    number={},
    pages={5503-5507},
    doi={10.1109/ICASSP43922.2022.9746438}
}

@inproceedings{Xu2019DBSCAN,
    author={Xu, Shuoyuan and Shin, Hyo-Sang and Tsourdos, Antonios},
    booktitle={2019 Workshop on Research, Education and Development of Unmanned Aerial Systems (RED UAS)}, 
    title={Distributed  Multi-Target  Tracking  with  {D-DBSCAN}  Clustering}, 
    year={2019},
    doi={10.1109/REDUAS47371.2019.8999712}
}

@article{Hyowon2020Cooperative,
    author={Kim, Hyowon and Granström, Karl and Gao, Lin and Battistelli, Giorgio and Kim, Sunwoo and Wymeersch, Henk},
    journal={IEEE Trans. Wirel. Commun.}, 
    title={{5G mmWave} Cooperative Positioning and Mapping Using Multi-Model PHD Filter and Map Fusion}, 
    year={2020},
    volume={19},
    number={6},
    pages={3782-3795},
    doi={10.1109/TWC.2020.2978479}
}

@article{Kim2023:SLAM,
    author={Kim, Hyowon and Chen, Hui and Keskin, Musa Furkan and Ge, Yu and Keykhosravi, Kamran and Alexandropoulos, George C. and Kim, Sunwoo and Wymeersch, Henk},
    journal={IEEE Trans. Wirel. Commun.}, 
    title={{RIS}-Enabled and Access-Point-Free Simultaneous Radio Localization and Mapping}, 
    year={2023},
    volume={},
    number={},
    pages={1-1},
    doi={10.1109/TWC.2023.3307455}
}

@article{Elzanaty2021,
    author={Elzanaty, Ahmed and Guerra, Anna and Guidi, Francesco and Alouini, Mohamed-Slim},
    journal={IEEE Trans. Signal Process.}, 
    title={Reconfigurable Intelligent Surfaces for Localization: Position and Orientation Error Bounds}, 
    year={2021},
    volume={69},
    number={},
    pages={5386-5402},
    doi={10.1109/TSP.2021.3101644}
}

@article{Schuhmacher2008:OSPA,
    author={Schuhmacher, Dominic and Vo, Ba-Tuong and Vo, Ba-Ngu},
    journal={IEEE Trans. Signal Process.}, 
    title={A Consistent Metric for Performance Evaluation of Multi-Object Filters}, 
    year={2008},
    volume={56},
    number={8},
    pages={3447-3457},
    doi={10.1109/TSP.2008.920469}
}

@article{Vo2019:GLMB,
    author={Vo, Ba-Ngu and Vo, Ba-Tuong and Beard, Michael},
    journal={IEEE Trans. Signal Process.}, 
    title={Multi-Sensor Multi-Object Tracking With the Generalized Labeled Multi-Bernoulli Filter}, 
    year={2019},
    volume={67},
    number={23},
    pages={5952-5967},
    doi={10.1109/TSP.2019.2946023}
}

@article{Zhang2022:MetaRadar,
    author={Zhang, Haobo and Zhang, Hongliang and Di, Boya and Bian, Kaigui and Han, Zhu and Song, Lingyang},
    journal={IEEE Trans. Wirel. Commun.}, 
    title={{MetaRadar}: Multi-Target Detection for Reconfigurable Intelligent Surface Aided Radar Systems}, 
    year={2022},
    volume={21},
    number={9},
    pages={6994-7010},
    doi={10.1109/TWC.2022.3153792}
}

@article{Meng2022:Sensing,
    author={Meng, Kaitao and Wu, Qingqing and Schober, Robert and Chen, Wen},
    journal={IEEE Trans. Commun.}, 
    title={Intelligent Reflecting Surface Enabled Multi-Target Sensing}, 
    year={2022},
    volume={70},
    number={12},
    pages={8313-8330},
    doi={10.1109/TCOMM.2022.3217564}
}

@article{Huang2023:Harnessing,
    author={Huang, Yixuan and Yang, Jie and Tang, Wankai and Wen, Chao-Kai and Xia, Shuqiang and Jin, Shi},
    journal={IEEE Trans. Wirel. Commun.}, 
    title={Joint Localization and Environment Sensing by Harnessing {NLOS} Components in {RIS}-aided {mmWave} Communication Systems}, 
    year={2023},
    volume={},
    number={},
    pages={1-1},
    doi={10.1109/TWC.2023.3266343}
}

@article{Tang2021:RIS,
    author={Tang, Wankai and Chen, Ming Zheng and Chen, Xiangyu and Dai, Jun Yan and Han, Yu and Di Renzo, Marco and Zeng, Yong and Jin, Shi and Cheng, Qiang and Cui, Tie Jun},
    journal={IEEE Trans. Wirel. Commun.}, 
    title={Wireless Communications With Reconfigurable Intelligent Surface: Path Loss Modeling and Experimental Measurement}, 
    year={2021},
    volume={20},
    number={1},
    pages={421-439},
    doi={10.1109/TWC.2020.3024887}
}

@article{He2023:WiFi,
    author={He, Ying and Zhang, Dongheng and Chen, Yan},
    journal={IEEE Internet Things J.}, 
    title={High-Resolution {WiFi} Imaging With Reconfigurable Intelligent Surfaces}, 
    year={2023},
    volume={10},
    number={2},
    pages={1775-1786},
    doi={10.1109/JIOT.2022.3210686}
}

@article{Hu2021:MetaSensing,
    author={Hu, Jingzhi and Zhang, Hongliang and Bian, Kaigui and Renzo, Marco Di and Han, Zhu and Song, Lingyang},
    journal={IEEE J. Sel. Areas Commun.}, 
    title={MetaSensing: Intelligent Metasurface Assisted {RF 3D} Sensing by Deep Reinforcement Learning}, 
    year={2021},
    volume={39},
    number={7},
    pages={2182-2197},
    doi={10.1109/JSAC.2021.3078492}
}

@article{Schmidt1986:MUSIC,
    author={R. Schmidt},
    journal={IEEE Trans. Antennas Propag.}, 
    title={Multiple emitter location and signal parameter estimation}, 
    year={1986},
    volume={34},
    number={3},
    pages={276-280},
    doi={10.1109/TAP.1986.1143830}
}

@article{Shan1985:Smoothing,
    author={Tie-Jun Shan and Wax, M. and Kailath, T.},
    journal={IEEE Trans. Acoust. Speech Signal Process.}, 
    title={On spatial smoothing for direction-of-arrival estimation of coherent signals}, 
    year={1985},
    volume={33},
    number={4},
    pages={806-811},
    doi={10.1109/TASSP.1985.1164649}
}

@article{Zhang2023:WiFi,
    author = {Zhang, Ganlin and Zhang, Dongheng and He, Ying and Chen, Jinbo and Zhou, Fang and Chen, Yan},
    year = {2023},
    month = {10},
    pages = {1-1},
    title = {Multi-Person Passive WiFi Indoor Localization With Intelligent Reflecting Surface},
    volume = {PP},
    journal = {IEEE Trans. Wirel. Commun.},
    doi = {10.1109/TWC.2023.3244369}
}

@book{Hua2023TwoStage,
    title = {{3D} Multi-Target Localization Via Intelligent Reflecting Surface: Protocol and Analysis},
    author = {Meng Hua and Guangji Chen and Shaodan Ma and Chau Yuen and Hing Cheung So},
    publisher = {arXiv},
    year = {2023},
}

@article{Guo2017Beamspace,
    author={Guo, Ziyu and Wang, Xiaodong and Heng, Wei},
    journal={IEEE Trans. Wirel. Commun.}, 
    title={Millimeter-Wave Channel Estimation Based on 2-D Beamspace {MUSIC} Method}, 
    year={2017},
    volume={16},
    number={8},
    pages={5384-5394},
    doi={10.1109/TWC.2017.2710049}
}

@article{Liu2022:Fundamental,
    author={Liu, An and Huang, Zhe and Li, Min and Wan, Yubo and Li, Wenrui and Han, Tony Xiao and Liu, Chenchen and Du, Rui and Tan, Danny Kai Pin and Lu, Jianmin and Shen, Yuan and Colone, Fabiola and Chetty, Kevin},
    journal={IEEE Commun. Surv. Tutor.}, 
    title={A Survey on Fundamental Limits of Integrated Sensing and Communication}, 
    year={2022},
    volume={24},
    number={2},
    pages={994-1034},
    doi={10.1109/COMST.2022.3149272}
}


@book{Spagnolini2018:Statistical,
    author = {Spagnolini, Umberto},
    publisher = {John Wiley \& Sons, Ltd},
    isbn = {9781119294016},
    title = {Statistical Signal Processing in Engineering},
    doi = {https://doi.org/10.1002/9781119294016.ch10},
    year = {2018},
}

@article{Sen2011:Sparsity,
    author={Sen, Satyabrata and Nehorai, Arye},
    journal={IEEE Trans. Signal Process.}, 
    title={Sparsity-Based Multi-Target Tracking Using {OFDM} Radar}, 
    year={2011},
    volume={59},
    number={4},
    pages={1902-1906},
    doi={10.1109/TSP.2010.2103064}
}

@book{Vaart1998:Asymptotic,
    place={Cambridge},
    series={Cambridge Series in Statistical and Probabilistic Mathematics},
    title={Asymptotic Statistics},
    publisher={Cambridge University Press},
    author={Vaart, A. W. van der},
    year={1998},
    collection={Cambridge Series in Statistical and Probabilistic Mathematics}
}

@book{Madsen2010:General,
  author = {Henrik Madsen and Poul Thyregod},
  edition = {1st ed.},
  publisher = {{CRC} press},
  title = {Introduction to general and generalized linear models},
  doi = {10.1201/9781439891148},
  year = 2010
}

@book{Tagliaferri2023:Cooperative,
    title={Cooperative Coherent Multistatic Imaging and Phase Synchronization in Networked Sensing}, 
    author={Dario Tagliaferri and Marco Manzoni and Marouan Mizmizi and Stefano Tebaldini and Andrea Virgilio Monti-Guarnieri and Claudio Maria Prati and Umberto Spagnolini},
    year={2023},
    publisher={arXiv},
}

@inproceedings{Lehmann2006:High,
    author={Lehmann, Nikolaus H. and Haimovich, Alexander M. and Blum, Rick S. and Cimini, Len},
    booktitle={2006 Fortieth Asilomar Conference on Signals, Systems and Computers}, 
    title={High Resolution Capabilities of MIMO Radar}, 
    year={2006},
    volume={},
    number={},
    pages={25-30},
    doi={10.1109/ACSSC.2006.356576}
}

@book{Stoica2005:Spectral,
    title={Spectral Analysis of Signals},
    author={Stoica, P. and Moses, R.L.},
    isbn={9780131139565},
    lccn={2004043191},
    year={2005},
    publisher={Pearson Prentice Hall}
}

@article{Stoica1989:MUSIC,
    author={Stoica, P. and Nehorai, Arye},
    journal={IEEE Trans. Acoust. Speech Signal Process.}, 
    title={MUSIC, maximum likelihood, and Cramer-Rao bound}, 
    year={1989},
    volume={37},
    number={5},
    pages={720-741},
    doi={10.1109/29.17564}
}

@article{Cui2021:Integrating,
    author={Cui, Yuanhao and Liu, Fan and Jing, Xiaojun and Mu, Junsheng},
    journal={IEEE Network}, 
    title={Integrating Sensing and Communications for Ubiquitous IoT: Applications, Trends, and Challenges}, 
    year={2021},
    volume={35},
    number={5},
    pages={158-167},
    doi={10.1109/MNET.010.2100152}
}

@article{Anderson1963:Asymptotic,
    author = {T. W. Anderson},
    title = {{Asymptotic Theory for Principal Component Analysis}},
    volume = {34},
    journal = {The Annals of Mathematical Statistics},
    number = {1},
    publisher = {Institute of Mathematical Statistics},
    pages = {122 -- 148},
    year = {1963},
    doi = {10.1214/aoms/1177704248}
}

@article{Crouse2016:Assignment,
    author={Crouse, David F.},
    journal={Trans. Aerosp. Electron. Syst.}, 
    title={On implementing {2D} rectangular assignment algorithms}, 
    year={2016},
    volume={52},
    number={4},
    pages={1679-1696},
    doi={10.1109/TAES.2016.140952}
}

@article{Emadi2018:OMP,
    title = {{OMP}-based {DOA} estimation performance analysis},
    journal = {Digital Signal Processing},
    volume = {79},
    pages = {57-65},
    year = {2018},
    issn = {1051-2004},
    doi = {https://doi.org/10.1016/j.dsp.2018.04.006},
    author = {Mohammad Emadi and Ehsan Miandji and Jonas Unger}
}

@inproceedings{Wymeersch2020:Detection,
    author={Wymeersch, Henk and Seco-Granados, Gonzalo},
    booktitle={2020 2nd 6G Wireless Summit (6G SUMMIT)}, 
    title={Adaptive Detection Probability for {mmWave 5G SLAM}}, 
    year={2020},
    volume={},
    number={},
    pages={1-5},
    doi={10.1109/6GSUMMIT49458.2020.9083898}
}

@book{Saggese2023:Control,
    author = {Fabio Saggese and Victor Croisfelt and Radosław Kotaba and Kyriakos Stylianopoulos and George C. Alexandropoulos and Petar Popovski},
    title = {A Framework for Control Channels Applied to Reconfigurable Intelligent Surfaces},
    publisher = {arXiv},
    year = {2023}
}

@article{An2022:Control,
    author={An, Jiancheng and Xu, Chao and Wu, Qingqing and Ng, Derrick Wing Kwan and Renzo, Marco Di and Yuen, Chau and Hanzo, Lajos},
    journal={IEEE Wirel. Commun.}, 
    title={Codebook-Based Solutions for Reconfigurable Intelligent Surfaces and Their Open Challenges}, 
    year={2022},
    volume={},
    number={},
    pages={1-8},
    doi={10.1109/MWC.010.2200312}
}

@article{Chepuri2023:Integrated,
    author={Chepuri, Sundeep Prabhakar and Shlezinger, Nir and Liu, Fan and Alexandropoulos, George C. and Buzzi, Stefano and Eldar, Yonina C.},
    journal={IEEE Signal Process. Mag.}, 
    title={Integrated Sensing and Communications With Reconfigurable Intelligent Surfaces: From signal modeling to processing}, 
    year={2023},
    volume={40},
    number={6},
    pages={41-62},
    doi={10.1109/MSP.2023.3279986}
}

@article{Xie2024:RIS,
    author={Xie, Zhuang and Wu, Linlong and Zhu, Jiahua and Lops, Marco and Huang, Xiaotao and Shankar, M. R. Bhavani},
    journal={IEEE Transactions on Signal Processing}, 
    title={RIS-Aided Radar for Target Detection: Clutter Region Analysis and Joint Active-Passive Design}, 
    year={2024},
    volume={72},
    number={},
    pages={1706-1723},
    doi={10.1109/TSP.2024.3371292}
}

@inproceedings{Sofotasios2014:Analytic,
    author={Paschalis Sofotasios and Mikko Valkama and Theodoros Tsifitsis and Yury Brychkov and Steven Freear and George Karagiannidis},
    title={Analytic Solutions to a {Marcum} {Q}-Function-Based Integral and Application in Energy Detection of Unknown Signals over Multipath Fading Channels},
    booktitle={9th Int. Conf. Cognitive Radio Oriented Wireless Networks},
    year={2014},
    doi={10.4108/icst.crowncom.2014.255383}
}

@article{Tropp2007:OMP,
    author={Tropp, Joel A. and Gilbert, Anna C.},
    journal={IEEE Trans. Inf. Theo.}, 
    title={Signal Recovery From Random Measurements Via Orthogonal Matching Pursuit}, 
    year={2007},
    volume={53},
    number={12},
    pages={4655-4666},
    doi={10.1109/TIT.2007.909108}
}

@article{Malioutov2005:Sparse,
    author={Malioutov, D. and Cetin, M. and Willsky, A.S.},
    journal={IEEE Trans. Signal Process.}, 
    title={A sparse signal reconstruction perspective for source localization with sensor arrays}, 
    year={2005},
    volume={53},
    number={8},
    pages={3010-3022},
    doi={10.1109/TSP.2005.850882}
}

@inproceedings{Rabaster2013:Ambiguity,
    author={Rabaste, Olivier and Savy, Laurent and Cattenoz, Mathieu and Guyvarch, Jean-Paul},
    booktitle={Int. Conf. Radar}, 
    title={Signal waveforms and range/angle coupling in coherent colocated MIMO radar}, 
    year={2013},
    volume={},
    number={},
    pages={157-162},
    doi={10.1109/RADAR.2013.6651977}
}

@article{Antonio2007:Ambiguity,
    author={San Antonio, Geoffrey and Fuhrmann, Daniel R. and Robey, Frank C.},
    journal={IEEE J. Sel. Top. Signal Process.},
    title={MIMO Radar Ambiguity Functions}, 
    year={2007},
    volume={1},
    number={1},
    pages={167-177},
    doi={10.1109/JSTSP.2007.897058}
}

@inproceedings{Rahmathullah2017:GOSPA,
    author={Rahmathullah, Abu Sajana and Garc\'ia-Fern\'andez, \'Angel F. and Svensson, Lennart},
    booktitle={2017 20th Int. Conf. Inf. Fusion}, 
    title={Generalized optimal sub-pattern assignment metric}, 
    publisher={IEEE},
    year={2017},
    volume={},
    number={},
    pages={1-8},
    doi={10.23919/ICIF.2017.8009645}
}
